Code-Switching Reveals Language Anchoring in Multilingual LLMs

Multilingual Large Language Models (MLLMs) are increasingly expected to handle Code-Switched (CS) inputs, yet mixing languages frequently degrades performance relative to source- or target-language monolingual counterparts. To understand this degradation, we use grammar-forced CS as a controlled diagnostic setting for locating CS representations relative to their source and target counterparts. We introduce Anchor Bias, a geometric measure that quantifies language anchoring, whether a CS hidden state aligns closer to its source or target language counterpart. Across diverse MLLMs, Anchor Bias reveals a consistent grammar-frame effect: source-framed CS stays source-anchored, whereas target-framed CS shifts target-ward and shows larger Question Answering (QA) degradation. Motivated by this representational pattern, we propose CANVAS (Contextual Anchor-based Neural Vector Alignment Steering), an inference-time intervention that extracts a source-side canvas from the input and softly steers target-language hidden states toward the source anchor during prefill. CANVAS consistently recovers QA F1 across MLLMs and CS conditions, showing that internal anchoring signals provide an actionable target for mitigating CS inference failures.

==> tables/anchor_bias_main.tex <==
% §4  Representational anchor bias — main Layer-AB pool.
% Uses AB-Upper_nrm for the same 10-model dense+MoE pool as Table 1.
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c r r r r r}
\toprule
\textbf{Model} & \textbf{Pool} & \textsc{GF-Src} & \textsc{GF-Tgt} & \textsc{Rand} & \textsc{Sel} & $\Delta_{\mathrm{GF}}$ \\
\midrule
Aya-Expanse-8B & Dense & \ENanchor{+0.300} & \TGTanchor{-0.220} & \ENanchor{+0.002} & \TGTanchor{-0.079} & $+0.520$ \\
Qwen3.5-4B & Dense & \ENanchor{+0.169} & \TGTanchor{-0.262} & \TGTanchor{-0.085} & \TGTanchor{-0.143} & $+0.431$ \\
Qwen3.5-9B & Dense & \ENanchor{+0.185} & \TGTanchor{-0.256} & \TGTanchor{-0.076} & \TGTanchor{-0.139} & $+0.441$ \\
Qwen3.5-27B & Dense & \ENanchor{+0.154} & \TGTanchor{-0.197} & \TGTanchor{-0.045} & \TGTanchor{-0.101} & $+0.351$ \\
Llama3.1-70B & Dense & \ENanchor{+0.257} & \TGTanchor{-0.225} & \TGTanchor{-0.010} & \TGTanchor{-0.093} & $+0.482$ \\
Llama3.3-70B & Dense & \ENanchor{+0.267} & \TGTanchor{-0.191} & \ENanchor{+0.016} & \TGTanchor{-0.065} & $+0.458$ \\
\midrule
Mixtral-8x7B & MoE & \ENanchor{+0.273} & \TGTanchor{-0.452} & \TGTanchor{-0.136} & \TGTanchor{-0.237} & $+0.725$ \\
Phi-3.5-MoE & MoE & \ENanchor{+0.248} & \TGTanchor{-0.300} & \TGTanchor{-0.051} & \TGTanchor{-0.134} & $+0.548$ \\
Qwen3-30B-A3B & MoE & \ENanchor{+0.393} & \TGTanchor{-0.081} & \ENanchor{+0.149} & \ENanchor{+0.048} & $+0.474$ \\
Qwen3.5-35B-A3B & MoE & \ENanchor{+0.225} & \TGTanchor{-0.214} & \TGTanchor{-0.020} & \TGTanchor{-0.086} & $+0.439$ \\
\midrule
\textit{Mean} & -- & $+0.247$ & $-0.240$ & $-0.026$ & $-0.103$ & $+0.487$ \\
\bottomrule
\end{tabular}}
\caption{%
  \textbf{Upper-layer normalized anchor bias across code-switching conditions.}
  Main anchor-bias tables report $\textsc{AB}^{upper}_{nrm}$: the upper-50\% layer average of question-content anchor bias after per-layer random-cosine normalization.
  Positive values indicate closer alignment to EN than TGT; negative values indicate closer alignment to TGT than EN.
  The same Layer-AB pool is used in Tables~\ref{tab:cs_grammar_forcing}, \ref{tab:anchor_bias_main}, and \ref{tab:layer_commitment}; q-pure/raw variants are moved to Appendix~\ref{tab:anchor_bias_variants}.
}
\label{tab:anchor_bias_main}
\end{table*}

==> tables/anchor_f1_correlation.tex <==
% §4  Anchor bias predicts performance degradation.
% Recomputed from the output CSVs for the 10-model Layer-AB pool.
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l c c c@{}}
\toprule
\textbf{Metric} & $n$ & $\rho$ & $p$ \\
\midrule
$\textsc{AB}_{q,nrm}$ (main) & 40 & $+0.485^{**}$ & 0.0015 \\
$\textsc{AB}^{upper}_{nrm}$ (upper-layer) & 40 & $+0.302^{\dagger}$ & 0.059 \\
\bottomrule
\end{tabular*}
\caption{%
  \textbf{Anchor bias predicts F1 degradation across model$\times$condition pairs.}
  Each point aggregates one $(\text{model},\text{CS condition})$ cell ($n{=}40$).
  Recomputing the correlation with the question-content normalized metric gives $\rho{=}+0.485$, matching the stronger value from the earlier q-pure analysis.
  The upper-layer aggregate is directionally consistent but weaker, so we report it as a robustness row.
  A positive $\rho$ means stronger EN anchoring corresponds to smaller F1 degradation.
  $^{\dagger}p{<}.10$; $^{**}p{<}.01$.
}
\label{tab:anchor_f1_correlation}
\end{table}


==> tables/grammar_experiment.tex <==
% §3  Grammar-forcing natural experiment — compact contrast view.
% Main anchor value is AB-Upper_nrm; model pool is 6 dense + 4 MoE with layer traces.
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.06}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l r r r r r r}
\toprule
\multirow{2}{*}{\textbf{Model}} &
  \multicolumn{3}{c}{\textbf{Upper-layer anchor contrast}} &
  \multicolumn{3}{c}{\textbf{F1 degradation}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & \textsc{GF-Src} & \textsc{GF-Tgt} & $\Delta_{\textsc{AB}}$ &
   \textsc{GF-Src} & \textsc{GF-Tgt} & $\Delta_{\textsc{drop}}$ \\
\midrule
Aya-Expanse-8B         & \ENanchor{+0.300} & \TGTanchor{-0.220} & $+0.520$ & $-2.3$ & $-4.9$ & $+2.6$ \\
Qwen3.5-4B             & \ENanchor{+0.169} & \TGTanchor{-0.262} & $+0.431$ & $-1.8$ & $-2.8$ & $+1.0$ \\
Qwen3.5-9B             & \ENanchor{+0.185} & \TGTanchor{-0.256} & $+0.441$ & $-1.2$ & $-5.0$ & $+3.8$ \\
Qwen3.5-27B            & \ENanchor{+0.154} & \TGTanchor{-0.197} & $+0.351$ & $-3.3$ & $-6.2$ & $+2.9$ \\
Llama3.1-70B           & \ENanchor{+0.257} & \TGTanchor{-0.225} & $+0.482$ & $-6.2$ & $-9.6$ & $+3.4$ \\
Llama3.3-70B           & \ENanchor{+0.267} & \TGTanchor{-0.191} & $+0.458$ & $-5.2$ & $-7.3$ & $+2.1$ \\
\midrule
Mixtral-8x7B           & \ENanchor{+0.273} & \TGTanchor{-0.452} & $+0.725$ & $-4.1$ & $-5.0$ & $+0.9$ \\
Phi-3.5-MoE            & \ENanchor{+0.248} & \TGTanchor{-0.300} & $+0.548$ & $-3.5$ & $-6.6$ & $+3.1$ \\
Qwen3-30B-A3B          & \ENanchor{+0.393} & \TGTanchor{-0.081} & $+0.474$ & $-2.4$ & $-4.7$ & $+2.3$ \\
Qwen3.5-35B-A3B        & \ENanchor{+0.225} & \TGTanchor{-0.214} & $+0.439$ & $-5.6$ & $-11.1$ & $+5.5$ \\
\midrule
\textit{Mean} & $+0.247$ & $-0.240$ & $+0.487$ & $-3.6$ & $-6.3$ & $+2.8$ \\
\bottomrule
\end{tabular}}
\caption{%
  \textbf{Grammar-forcing creates a relative anchoring and performance contrast.}
  This table uses the unified \emph{Layer-AB pool}: six dense models and four MoE models for which upper-layer traces are available.
  $\Delta_{\textsc{AB}}=\textsc{AB}^{upper}_{nrm}(\textsc{GF-Src})-\textsc{AB}^{upper}_{nrm}(\textsc{GF-Tgt})$;
  positive values mean source-structured code-switching is relatively more EN-like, or less TGT-like, than target-structured code-switching.
  $\Delta_{\textsc{drop}}=\Delta\text{F1}_{\textsc{GF-Src}}-\Delta\text{F1}_{\textsc{GF-Tgt}}$;
  positive values mean \textsc{GF-Src} loses less F1 than \textsc{GF-Tgt}.
  The claim is relative separation, not that every \textsc{GF-Src} value must be positive in absolute sign.
}
\label{tab:cs_grammar_forcing}
\end{table}

==> tables/language.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
\multirow{2}{*}{\textbf{Group}} &
\multicolumn{3}{c}{\textbf{Anchor bias}} &
\multicolumn{3}{c}{$\boldsymbol{\Delta}$\textbf{F1}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& \textsc{GF-Src} & \textsc{GF-Tgt} & $\Delta_{\mathrm{AB}}$
& \textsc{GF-Src} & \textsc{GF-Tgt} & $\Delta_{\mathrm{drop}}$ \\
\midrule
SVO & $+0.051$ & $-0.128$ & $+0.180$ & $-1.6$ & $-5.2$ & $+3.6$ \\
SOV & $+0.003$ & $-0.185$ & $+0.188$ & $-4.6$ & $-7.1$ & $+2.5$ \\
\bottomrule
\end{tabular}}
\caption{\textbf{Word-order grouped breakdown.}
SVO includes Spanish, French, and Chinese; SOV includes Bengali, Hindi, Korean, Marathi, Urdu, and Toba Batak. Both groups preserve the same direction: \textsc{GF-Src} is more EN-anchored and less damaging than \textsc{GF-Tgt}.}
\label{tab:word_order_breakdown}
\end{table}

==> tables/layer_analysis.tex <==
% §4  Compact layer-wise language commitment.
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c r r r}
\toprule
\textbf{Model} & \textbf{Pool} & \textsc{GF-Src} & \textsc{GF-Tgt} & $\Delta$ \\
\midrule
Aya-Expanse-8B & Dense & 85.6 & 42.8 & +42.8 \\
Qwen3.5-4B & Dense & 70.7 & 29.2 & +41.5 \\
Qwen3.5-9B & Dense & 72.9 & 32.5 & +40.4 \\
Qwen3.5-27B & Dense & 73.5 & 34.4 & +39.1 \\
Llama3.1-70B & Dense & 80.6 & 38.0 & +42.6 \\
Llama3.3-70B & Dense & 81.4 & 39.5 & +41.9 \\
\midrule
Mixtral-8x7B & MoE & 74.6 & 33.2 & +41.4 \\
Phi-3.5-MoE & MoE & 64.8 & 31.7 & +33.1 \\
Qwen3-30B-A3B & MoE & 78.5 & 42.1 & +36.4 \\
Qwen3.5-35B-A3B & MoE & 74.3 & 37.5 & +36.8 \\
\midrule
\textit{Mean} & -- & 75.7 & 36.1 & +39.6 \\
\bottomrule
\end{tabular}}
\caption{%
  \textbf{Upper-layer commitment is stronger under source-structured CS.}
  Entries are the percentage of layers with positive question-content anchor bias after per-layer normalization.
  The compact table reports the grammar contrast only; full condition-level anchor values are in Table~\ref{tab:anchor_bias_main}.
}
\label{tab:layer_commitment}
\end{table}


==> tables/moe_routing.tex <==
% §5  MoE routing-level evidence.
% Values regenerated from outputs_recombined.zip.
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4.4pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c r r r r}
\toprule
\textbf{Model} & \textbf{Cond} & \textbf{Jac-EN} & \textbf{Jac-TGT} & \textbf{RB} & $d$ \\
\midrule
  \multirow{4}{*}{\shortstack[l]{Phi-3.5-MoE\\(16 exp./layer)}} & \textsc{GF-Src} & 0.969 & 0.960 & $\mathbf{+0.008}_{\scriptscriptstyle\mathrm{EN}}$ & \multirow{4}{*}{0.99} \\
   & \textsc{GF-Tgt} & 0.960 & 0.967 & \underline{$-0.007_{\scriptscriptstyle\mathrm{TGT}}$} &  \\
   & \textsc{Rand} & 0.963 & 0.964 & $-0.001_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
   & \textsc{Sel} & 0.961 & 0.964 & $-0.003_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
\midrule
  \multirow{4}{*}{\shortstack[l]{Qwen3-30B-A3B\\(128 exp./layer)}} & \textsc{GF-Src} & 0.910 & 0.897 & $+0.013_{\scriptscriptstyle\mathrm{EN}}$ & \multirow{4}{*}{1.37} \\
   & \textsc{GF-Tgt} & 0.886 & 0.917 & $\mathbf{-0.031}_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
   & \textsc{Rand} & 0.894 & 0.907 & $-0.013_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
   & \textsc{Sel} & 0.892 & 0.911 & \underline{$-0.019_{\scriptscriptstyle\mathrm{TGT}}$} &  \\
\midrule
  \multirow{4}{*}{\shortstack[l]{Qwen3.5-35B-A3B\\(256 exp./layer)}} & \textsc{GF-Src} & 0.835 & 0.806 & \underline{$+0.030_{\scriptscriptstyle\mathrm{EN}}$} & \multirow{4}{*}{1.41} \\
   & \textsc{GF-Tgt} & 0.804 & 0.836 & $\mathbf{-0.032}_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
   & \textsc{Rand} & 0.816 & 0.823 & $-0.007_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
   & \textsc{Sel} & 0.812 & 0.827 & $-0.015_{\scriptscriptstyle\mathrm{TGT}}$ &  \\
\bottomrule
\end{tabular}}
\caption{%
  \textbf{MoE expert routing bias mirrors representational anchoring.}
  Jac-EN/Jac-TGT are Jaccard overlaps between top-$k$ experts activated by CS and EN/TGT inputs.
  \textbf{RB}$=$Jac-EN$-$Jac-TGT is the routing analogue of anchor bias: positive values indicate EN-like routing and negative values indicate TGT-like routing.
  $d$ is Cohen's $d$ contrasting \textsc{GF-Src} vs.\ \textsc{GF-Tgt}; $d{>}0.8$ is large.
  \textbf{Bold}/\underline{underline} mark the largest/second-largest absolute RB per model.
}
\label{tab:moe_routing_bias}
\end{table}


==> tables/tab_alpha_distribution.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.8pt}
\begin{tabular}{lrrrrrrrr}
\toprule
Condition & Mean $\alpha$ & Std. & P10 & P50 & P90 & $\alpha{=}0.15$ & $\alpha{=}0.95$ & Mean $\gamma$ \\
\midrule
GF\_Src & 0.731 & 0.194 & 0.444 & 0.750 & 0.950 & 0.5 & 21.8 & 0.020 \\
GF\_Tgt & 0.546 & 0.218 & 0.243 & 0.547 & 0.817 & 4.4 & 3.6 & -0.125 \\
Random & 0.622 & 0.210 & 0.331 & 0.640 & 0.922 & 1.6 & 8.4 & 0.069 \\
Selective & 0.592 & 0.214 & 0.295 & 0.600 & 0.884 & 2.4 & 6.2 & 0.091 \\
\midrule
All & 0.622 & 0.220 & 0.310 & 0.648 & 0.950 & 2.2 & 10.0 & 0.066 \\
\bottomrule
\end{tabular}
\caption{\textbf{Full-run $\alpha$ distribution.} The clip range is active but not dominant: only a small fraction hits the lower bound, while the upper bound prevents high-confidence EN-anchored examples from becoming a full replacement operation.}
\label{tab:app_alpha_distribution}
\end{table}


==> tables/tab_high_src_ratio_examples.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.04}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}llllrrrll@{}}
\toprule
\textbf{Outcome} & \textbf{Model} & \textbf{Lang.} & \textbf{CS question} & $\rho_{\mathrm{SRC}}$ & $\alpha$ & \textbf{Base/CANVAS F1} & \textbf{Base} & \textbf{CANVAS} \\
\midrule
Fixed & \modelwithlogo{meta}{Llama3.1-70B} & Korean & What 성 overlooked Carmel Glen과 its burn and was situated in Knockentiber, East Ayrshire? & 0.90 & 0.52 & 0/50 & Barony of Knockentiber & Dean Castle \\
Fixed & \modelwithlogo{meta}{Llama3.3-70B} & Korean & What 성 overlooked Carmel Glen과 its burn and was situated in Knockentiber, East Ayrshire? & 0.90 & 0.57 & 0/50 & Barjarg Tower & Dean Castle \\
Fixed & \modelwithlogo{qwen}{Qwen3.5-9B} & Urdu & Which digits of the forefeet کے are vestigial اور tiny on the Isoodon obesulus? & 0.90 & 0.28 & 0/33 & Second and third & Digits 2 and 3 \\
Preserved & \modelwithlogo{qwen}{Qwen3.5-9B} & Simplified Chinese & From which 南美 university did Sergio Fajardo Valderrama receive his 数学 M.Sc.?  & 0.96 & 0.61 & 100/100 & Universidad de los Andes & Universidad de los Andes \\
Preserved & \modelwithlogo{qwen}{Qwen3.5-27B} & Simplified Chinese & From which 南美 university did Sergio Fajardo Valderrama receive his 数学 M.Sc.?  & 0.96 & 0.53 & 100/100 & Universidad de los Andes & Universidad de los Andes \\
Preserved & \modelwithlogo{qwen}{Qwen3.6-35B-A3B} & Simplified Chinese & From which 南美 university did Sergio Fajardo Valderrama receive his 数学 M.Sc.?  & 0.96 & 0.36 & 100/100 & Universidad de los Andes & Universidad de los Andes \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Source-heavy examples.}
Representative high-$\rho_{\mathrm{SRC}}$ cases show that CANVAS preserves direct CS answers and can still recover missed answers even when the input is mostly source-language text.}
\label{tab:app_high_src_ratio_examples}
\end{table*}


==> tables/tab_routing_similarity.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.04}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
\multirow{3}{*}{\raisebox{-1.3ex}{\textbf{Model}}} &
\multicolumn{6}{c}{\textbf{Cosine similarity over expert-frequency vectors}} &
\multicolumn{6}{c}{\textbf{Jaccard overlap over active expert sets}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
&
\multicolumn{3}{c}{$\cos(\mathrm{SRC},\mathrm{CS})$} &
\multicolumn{3}{c}{$\cos(\mathrm{TGT},\mathrm{CS})$} &
\multicolumn{3}{c}{$\mathrm{Jacc}(\mathrm{SRC},\mathrm{CS})$} &
\multicolumn{3}{c}{$\mathrm{Jacc}(\mathrm{TGT},\mathrm{CS})$} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\cmidrule(lr){8-10} \cmidrule(lr){11-13}
&
\cellcolor{SRCAnchor!18}\textsc{GF-Src} & \textsc{GF-Tgt} & $d$ &
\textsc{GF-Src} & \cellcolor{TGTAnchor!18}\textsc{GF-Tgt} & $d$ &
\cellcolor{SRCAnchor!18}\textsc{GF-Src} & \textsc{GF-Tgt} & $d$ &
\textsc{GF-Src} & \cellcolor{TGTAnchor!18}\textsc{GF-Tgt} & $d$ \\
\midrule
\modelwithlogo{qwen}{Qwen3-30B-A3B}
& 0.924 & 0.879 & +0.64
& 0.912 & 0.943 & -0.49
& 0.910 & 0.886 & +0.94
& 0.897 & 0.917 & -0.68 \\

\modelwithlogo{qwen}{Qwen3.6-35B-A3B}
& 0.933 & 0.905 & +0.63
& 0.925 & 0.944 & -0.40
& 0.646 & 0.586 & +0.56
& 0.596 & 0.653 & -0.53 \\

\modelwithlogo{microsoft}{Phi-3.5-MoE}
& 0.896 & 0.843 & +0.55
& 0.905 & 0.942 & -0.51
& 0.969 & 0.960 & +0.65
& 0.960 & 0.967 & -0.42 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Routing similarity under grammar-forced CS.}
We use the same routing metric and layout as Table~\ref{tab:routing}. Highlighted columns indicate the frame-matched route; $d$ reports the standardized gap between \textsc{GF-Src} and \textsc{GF-Tgt}.}
\label{tab:app_routing_similarity}
\end{table*}

